RyBench: Runtime Verification Benchmarking Framework over Publish/Subscribe Networks

Autonomous systems built as distributed, node-based systems communicate via publish/subscribe middleware. Runtime Verification (RV) tools are used to monitor those systems against formal specifications, receiving monitored events through the pub/sub channel. An RV tool's practical value depends on its monitoring throughput capacity and verdict latency, besides its correctness, so a systematic benchmarking setup is needed to evaluate how efficiently these tools run. This paper presents RyBench, a pub/sub-based benchmarking framework that acts as a synthetic event publisher in place of a monitored system, providing a common benchmarking setup. RyBench separates benchmark generation, serialization, and transport into distinct components, enabling the combination of different event-generation strategies, data formats, and transport layers. We also evaluate the framework's throughput capacity across these configurations using Open Simulation Interface (OSI) schemas and Timescales properties, and illustrate the end-to-end benchmarking flow through an application to Reelay and an integration with MonPoly.

==> eptcsdata.tex <==
\providecommand{\firstpage}{72}
\providecommand{\publicationstatus}{Matt Luckcuck, Maike Schwammberger, \& Akhila Bairy (Eds.):\\
Eighth International Workshop on Formal Methods\\
for Autonomous Systems (FMAS 2026)\\
EPTCS 457, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.457.6}{10.4204/EPTCS.457.6}}
\pdfoutput=1

